What killed the Convex Booster ?

A landmark negative result of Long and Servedio established a worst-case spectacular failure of a supervised learning trio (loss, algorithm, model) otherwise praised for its high precision machinery. Hundreds of papers followed up on the two suspected culprits: the loss (for being convex) and/or the algorithm (for fitting a classical boosting blueprint). Here, we call to the half-century+ founding theory of losses for class probability estimation (properness), an extension of Long and Servedio's results and a new general boosting algorithm to demonstrate that the real culprit in their specific context was in fact the (linear) model class. We advocate for a more general stanpoint on the problem as we argue that the source of the negative result lies in the dark side of a pervasive -- and otherwise prized -- aspect of ML: \textit{parameterisation}.

==> content-arxiv/conclusion.tex <==

\section{Conclusion}\label{sec-conc}

In this paper, we have used the founding theory of losses for class
probability estimation (properness) and a new boosting algorithm to demonstrate that the source of the negative result in the context of Long and Servedio's results is the model class. More than shining a new light on the model class' "responsibility" for the negative result, we believe our results rather show pitfalls of general parameterisations of a ML problem, including model class but also the learning algorithm and the loss function it optimizes. It remains an open question as to whether such stark "breakdowns" can be shown for highly ML-relevant triples (algorithm, loss, model) different from ours / \cite{lsRC}.
